Control of Generalized Energy Storage Networks

The integration of intermittent and volatile renewable energy resources requires increased flexibility in the operation of the electric grid. Storage, broadly speaking, provides the flexibility of shifting energy over time; network, on the other hand, provides the flexibility of shifting energy over geographical locations. The optimal control of general storage networks in uncertain environments is an important open problem. The key challenge is that, even in small networks, the corresponding constrained stochastic control problems with continuous spaces suffer from curses of dimensionality, and are intractable in general settings. For large networks, no efficient algorithm is known to give optimal or near-optimal performance. This paper provides an efficient and provably near-optimal algorithm to solve this problem in a very general setting. We study the optimal control of generalized storage networks, i.e., electric networks connected to distributed generalized storages. Here generalized storage is a unifying dynamic model for many components of the grid that provide the functionality of shifting energy over time, ranging from standard energy storage devices to deferrable or thermostatically controlled loads. An online algorithm is devised for the corresponding constrained stochastic control problem based on the theory of Lyapunov optimization. We prove that the algorithm is near-optimal, and construct a semidefinite program to min- imize the sub-optimality bound. The resulting bound is a constant that depends only on the parameters of the storage network and cost functions, and is independent of uncertainty realizations. Numerical examples are given to demonstrate the effectiveness of the algorithm.

==> networkStorageResults-conf.tex <==
\section{Results for Networked Systems}\label{sec:networkResults}
For completeness, we provide a summary of results for networks with more than one buses and storages; detailed discussions and proofs can be found in \cite{QCYR:report}. For each bus $v\in \V$, we use $X_v$ to denote the corresponding variable $X$ defined for single bus systems in Section~\ref{sec:proofSingleBus}, and $\mathbf{X}$ to denote the vector $\{X_v\}_{v\in \V}$. The online optimization, which corresponds to \Pk{3} in the single bus systems, is as stated in \eqref{prob:P3_network}. Suppose that Assumption~\ref{assume:singleBusProof} is in force for each bus $v\in \V$. 
The following results hold for the control sequence $(\un^\star(\Pk{3}),\fn^\star(\Pk{3}))$ obtained from Algorithm~\ref{alg}.
\begin{theorem}[Feasibility]
Suppose the initial storage level satisfies $\b_v(1) \in [\bmin_v, \bmax_v]$, for all $v\in\V$, then the storage level sequence $\{\bn(t): t\ge 1 \}$ induced by the sequence of storage operation $(\un^\star(\Pk{3}))$ is feasible with respect to storage level constraints, \ie, $\b_v(t) \in [\bmin_v, \bmax_v]$ for all $t$ and $v\in\V$, provided that
\[
\ksmin_v\le  \ks_v \le \ksmax_v,\,\,0 < \W  \le \Wmax_v, 
\]
for all $v\in \V$.
\end{theorem}
\begin{theorem} [Performance]\label{thm:perf_lyap}
The sub-optimality of control sequence $(\un^\star(\Pk{3}),\fn^\star(\Pk{3}))$ is bounded by $\M(\ksn)/\W$, that is
\begin{equation*}\label{eq:networkiidperf_bdd}
\Jk{1}^\star\! \le\!  \Jk{1}(\un^\star(\Pk{3}),\fn^\star(\Pk{3})) \!\le\! \Jk{1}^\star + \frac{\M(\ksn)}{\W},
\end{equation*}
%Let $\uhat(t)$ be the control action chosen by solving \textbf{P3} and
%\[
%\begin{split}
%\Jk{3}^\star(t)=&\sum_{\ell = 1}^L \p(t, \ell) \Bigg(\alI(\ell) \d(t) - \alC(\ell)\hC\left( \pos{\uhat(t)}\right) \\
%&\quad + \alD(\ell) \hD\left(\neg{\uhat(t)}\right) + \alConst(\ell)\Bigg)^+.
%\end{split}
%\]
%Then
% \begin{equation} \label{eq:perf_bdd}
%  \lim_{T \to \infty} \frac{1}{T}\expec \left[ \sum_{t=1}^{T} \Jk{3}^\star(t)\right]  \leq \Jk{1}^\star + \frac{\M(\ks) }{\W}.
%\end{equation}
where
\[
\M(\ksn)=\Mone(\ksn)+\Mtwo(\ksn)\label{eq:M:network},
\]
\[
\Mone(\ksn) =\sum_{v\in\V}\Mone_v(\ks_v),
\]
and
\[
\Mtwo(\ksn) =\sum_{v\in\V}\la_v (1-\la_v)\Mtwo_v(\ks_v).
\]
\end{theorem}
The semidefinite program for minimizing the bound is as follows.
\begin{lemma}[Semidefinite Optimization of ${\M(\ksn)}/{\W}$]
Let symmetric positive definite matrices $\Xumin_v$, $\Xumax_v$, $\Xbmin_v$, and $\Xbmax_v$, $v\in\V$, be defined as follows
\begin{equation*}
\!\!\Xudot_v\!\! = \!\!\begin{bmatrix}
\None_v&\!\!\udot_v+(1-\la_v)\ks_v\\
*& 2\W
\end{bmatrix}, \,\,
\Xbdot_v\!\! = \!\!\begin{bmatrix}
\Ntwo_v&\!\!\bdot_v+\ks_v\\
*& \W
\end{bmatrix},\!\!
\end{equation*}
where $(\cdot)$ can be either $\max$ or $\min$, and $\None_v$ and $\Ntwo_v$ are auxiliary variables, for any $v\in\V$. Then the sub-optimality bound $\M(\ksn)/\W$ can be optimized by solving the following semidefinite program
\begin{subequations}\label{prob:sdp_network}
\begin{align}
\emph{\minimize} \quad & \sum_{v\in\V}\None_{v}+\la_v(1-\la_v)\Ntwo_v \\
\emph{\st} \quad & \ksmin_v\le  \ks_v \le \ksmax_v, \label{c1}\\
& 0 <  \W  \le \Wmax_v, \\
& \Xumin_v,\Xumax_v, \Xbmin_v, \Xbmax_v \succeq 0,\label{cend}
\end{align}
\end{subequations}
where constraints \eqref{c1}-\eqref{cend} hold for all $v\in \V$. 
\end{lemma}


